Depth Contrast: Self-Supervised Pretraining on 3DPM Images for Mining Material Classification

This work presents a novel self-supervised representation learning method to learn efficient representations without labels on images from a 3DPM sensor (3-Dimensional Particle Measurement; estimates the particle size distribution of material) utilizing RGB images and depth maps of mining material on the conveyor belt. Human annotations for material categories on sensor-generated data are scarce and cost-intensive. Currently, representation learning without human annotations remains unexplored for mining materials and does not leverage on utilization of sensor-generated data. The proposed method, Depth Contrast, enables self-supervised learning of representations without labels on the 3DPM dataset by exploiting depth maps and inductive transfer. The proposed method outperforms material classification over ImageNet transfer learning performance in fully supervised learning settings and achieves an F1 score of 0.73. Further, The proposed method yields an F1 score of 0.65 with an 11% improvement over ImageNet transfer learning performance in a semi-supervised setting when only 20% of labels are used in fine-tuning. Finally, the Proposed method showcases improved performance generalization on linear evaluation. The implementation of proposed method is available on GitHub.

==> tables/classwise_EXP1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\centering
\caption{Classwise precision, recall and F1 score for Experiment 1 }
\label{tab:my-table}
\begin{tabular}{|c|c|c|l|l|l|l|l|l|l|}
\hline
\textbf{Classes} & \textbf{Set} & \textbf{Metric} & \multicolumn{1}{c|}{\textbf{Mixed1}} & \multicolumn{1}{c|}{\textbf{Agglomerated}} & \multicolumn{1}{c|}{\textbf{Mixed2}} & \multicolumn{1}{c|}{\textbf{Ore1}} & \multicolumn{1}{c|}{\textbf{Ore2}} & \multicolumn{1}{c|}{\textbf{Ore3}} & \multicolumn{1}{c|}{\textbf{Cylindrical}} \\ \hline
 &  & \textbf{Precision} & {\color[HTML]{1E1E1E} 0.31 ± 0.0235} & {\color[HTML]{1E1E1E} 0.65 ± 0.0755} & {\color[HTML]{1E1E1E} 0.70 ± 0.2032} & {\color[HTML]{1E1E1E} 0.89 ± 0.0185} & {\color[HTML]{1E1E1E} 0.89 ± 0.0721} & {\color[HTML]{1E1E1E} 0.69 ± 0.0768} & {\color[HTML]{1E1E1E} 0.75 ± 0.1912} \\ \cline{3-10} 
 &  & \textbf{Recall} & {\color[HTML]{1E1E1E} 0.63 ± 0.1522} & {\color[HTML]{1E1E1E} 0.84 ± 0.0166} & {\color[HTML]{1E1E1E} 0.23 ± 0.0405} & {\color[HTML]{1E1E1E} 0.72 ± 0.0527} & {\color[HTML]{1E1E1E} 0.72 ± 0.0433} & {\color[HTML]{1E1E1E} 0.71 ± 0.0450} & {\color[HTML]{1E1E1E} 0.58 ± 0.0859} \\ \cline{3-10} 
 & \multirow{-3}{*}{\textbf{Train}} & \textbf{F1} & {\color[HTML]{1E1E1E} 0.41 ± 0.0457} & {\color[HTML]{1E1E1E} 0.73 ± 0.0539} & {\color[HTML]{1E1E1E} 0.34 ± 0.0488} & {\color[HTML]{1E1E1E} 0.79 ± 0.0320} & {\color[HTML]{1E1E1E} 0.79 ± 0.0371} & {\color[HTML]{1E1E1E} 0.70 ± 0.0528} & {\color[HTML]{1E1E1E} 0.64 ± 0.0908} \\ \cline{2-10} 
 &  & \textbf{Precision} & {\color[HTML]{1E1E1E} 0.31 ± 0.0589} & {\color[HTML]{1E1E1E} 0.64 ± 0.0499} & {\color[HTML]{1E1E1E} 0.63 ± 0.3924} & {\color[HTML]{1E1E1E} 0.89 ± 0.0113} & {\color[HTML]{1E1E1E} 0.89 ± 0.0841} & {\color[HTML]{1E1E1E} 0.69 ± 0.0744} & {\color[HTML]{1E1E1E} 0.84 ± 0.1570} \\ \cline{3-10} 
 &  & \textbf{Recall} & {\color[HTML]{1E1E1E} 0.61 ± 0.1846} & {\color[HTML]{1E1E1E} 0.84 ± 0.0425} & {\color[HTML]{1E1E1E} 0.22 ± 0.1996} & {\color[HTML]{1E1E1E} 0.72 ± 0.0537} & {\color[HTML]{1E1E1E} 0.71 ± 0.0284} & {\color[HTML]{1E1E1E} 0.70 ± 0.0584} & {\color[HTML]{1E1E1E} 0.62 ± 0.2558} \\ \cline{3-10} 
\multirow{-6}{*}{\textbf{EfficientNet}} & \multirow{-3}{*}{\textbf{Test}} & \textbf{F1} & {\color[HTML]{1E1E1E} 0.40 ± 0.0643} & {\color[HTML]{1E1E1E} 0.72 ± 0.0203} & {\color[HTML]{1E1E1E} 0.29 ± 0.2164} & {\color[HTML]{1E1E1E} 0.80 ± 0.0294} & {\color[HTML]{1E1E1E} 0.79 ± 0.0300} & {\color[HTML]{1E1E1E} 0.69 ± 0.0610} & {\color[HTML]{1E1E1E} 0.67 ± 0.2046} \\ \hline
 &  & \textbf{Precision} & {\color[HTML]{1E1E1E} 0.38 ± 0.0468} & {\color[HTML]{1E1E1E} 0.88 ± 0.0506} & {\color[HTML]{1E1E1E} 0.56 ± 0.1884} & {\color[HTML]{1E1E1E} 0.79 ± 0.0976} & {\color[HTML]{1E1E1E} 0.88 ± 0.0621} & {\color[HTML]{1E1E1E} 0.52 ± 0.1634} & {\color[HTML]{1E1E1E} 0.94 ± 0.0395} \\ \cline{3-10} 
 &  & \textbf{Recall} & {\color[HTML]{1E1E1E} 0.53 ± 0.1321} & {\color[HTML]{1E1E1E} 0.78 ± 0.0377} & {\color[HTML]{1E1E1E} 0.40 ± 0.2056} & {\color[HTML]{1E1E1E} 0.79 ± 0.0629} & {\color[HTML]{1E1E1E} 0.77 ± 0.0423} & {\color[HTML]{1E1E1E} 0.59 ± 0.2200} & {\color[HTML]{1E1E1E} 0.70 ± 0.0393} \\ \cline{3-10} 
 & \multirow{-3}{*}{\textbf{Train}} & \textbf{F1} & {\color[HTML]{1E1E1E} 0.43 ± 0.0299} & {\color[HTML]{1E1E1E} 0.83 ± 0.0205} & {\color[HTML]{1E1E1E} 0.40 ± 0.1169} & {\color[HTML]{1E1E1E} 0.78 ± 0.0255} & {\color[HTML]{1E1E1E} 0.82 ± 0.0267} & {\color[HTML]{1E1E1E} 0.55 ± 0.1860} & {\color[HTML]{1E1E1E} 0.80 ± 0.0223} \\ \cline{2-10} 
 &  & \textbf{Precision} & {\color[HTML]{1E1E1E} 0.36 ± 0.0260} & {\color[HTML]{1E1E1E} 0.85 ± 0.0295} & {\color[HTML]{1E1E1E} 0.57 ± 0.1418} & {\color[HTML]{1E1E1E} 0.78 ± 0.1063} & {\color[HTML]{1E1E1E} 0.88 ± 0.0573} & {\color[HTML]{1E1E1E} 0.50 ± 0.1879} & {\color[HTML]{1E1E1E} 0.93 ± 0.1011} \\ \cline{3-10} 
 &  & \textbf{Recall} & {\color[HTML]{1E1E1E} 0.52 ± 0.1388} & {\color[HTML]{1E1E1E} 0.78 ± 0.0696} & {\color[HTML]{1E1E1E} 0.38 ± 0.2443} & {\color[HTML]{1E1E1E} 0.79 ± 0.0585} & {\color[HTML]{1E1E1E} 0.76 ± 0.0761} & {\color[HTML]{1E1E1E} 0.58 ± 0.2696} & {\color[HTML]{1E1E1E} 0.69 ± 0.1988} \\ \cline{3-10} 
\multirow{-6}{*}{\textbf{DenseNet}} & \multirow{-3}{*}{\textbf{Test}} & \textbf{F1} & {\color[HTML]{1E1E1E} 0.42 ± 0.0466} & {\color[HTML]{1E1E1E} 0.81 ± 0.0278} & {\color[HTML]{1E1E1E} 0.40 ± 0.1858} & {\color[HTML]{1E1E1E} 0.78 ± 0.0325} & {\color[HTML]{1E1E1E} 0.81 ± 0.0497} & {\color[HTML]{1E1E1E} 0.53 ± 0.2203} & {\color[HTML]{1E1E1E} 0.77 ± 0.1322} \\ \hline
 &  & \textbf{Precision} & {\color[HTML]{1E1E1E} 0.37 ± 0.0834} & {\color[HTML]{1E1E1E} 0.70 ± 0.1128} & {\color[HTML]{1E1E1E} 0.57 ± 0.1504} & {\color[HTML]{1E1E1E} 0.86 ± 0.0662} & {\color[HTML]{1E1E1E} 0.96 ± 0.0169} & {\color[HTML]{1E1E1E} 0.61 ± 0.0494} & {\color[HTML]{1E1E1E} 0.90 ± 0.1082} \\ \cline{3-10} 
 &  & \textbf{Recall} & {\color[HTML]{1E1E1E} 0.65 ± 0.1288} & {\color[HTML]{1E1E1E} 0.85 ± 0.0213} & {\color[HTML]{1E1E1E} 0.48 ± 0.0899} & {\color[HTML]{1E1E1E} 0.70 ± 0.0543} & {\color[HTML]{1E1E1E} 0.46 ± 0.2168} & {\color[HTML]{1E1E1E} 0.90 ± 0.0197} & {\color[HTML]{1E1E1E} 0.66 ± 0.1128} \\ \cline{3-10} 
 & \multirow{-3}{*}{\textbf{Train}} & \textbf{F1} & {\color[HTML]{1E1E1E} 0.46 ± 0.0299} & {\color[HTML]{1E1E1E} 0.76 ± 0.0771} & {\color[HTML]{1E1E1E} 0.51 ± 0.0650} & {\color[HTML]{1E1E1E} 0.77 ± 0.0331} & {\color[HTML]{1E1E1E} 0.60 ± 0.2006} & {\color[HTML]{1E1E1E} 0.73 ± 0.0321} & {\color[HTML]{1E1E1E} 0.75 ± 0.0833} \\ \cline{2-10} 
 &  & \textbf{Precision} & {\color[HTML]{1E1E1E} 0.33 ± 0.0481} & {\color[HTML]{1E1E1E} 0.68 ± 0.1119} & {\color[HTML]{1E1E1E} 0.54 ± 0.1702} & {\color[HTML]{1E1E1E} 0.84 ± 0.0486} & {\color[HTML]{1E1E1E} 0.93 ± 0.0819} & {\color[HTML]{1E1E1E} 0.60 ± 0.0746} & {\color[HTML]{1E1E1E} 0.95 ± 0.1220} \\ \cline{3-10} 
 &  & \textbf{Recall} & {\color[HTML]{1E1E1E} 0.64 ± 0.1490} & {\color[HTML]{1E1E1E} 0.84 ± 0.0520} & {\color[HTML]{1E1E1E} 0.44 ± 0.1877} & {\color[HTML]{1E1E1E} 0.68 ± 0.0860} & {\color[HTML]{1E1E1E} 0.45 ± 0.2762} & {\color[HTML]{1E1E1E} 0.87 ± 0.0351} & {\color[HTML]{1E1E1E} 0.67 ± 0.2079} \\ \cline{3-10} 
\multirow{-6}{*}{\textbf{ResNeXtNet}} & \multirow{-3}{*}{\textbf{Test}} & \textbf{F1} & {\color[HTML]{1E1E1E} 0.43 ± 0.0116} & {\color[HTML]{1E1E1E} 0.75 ± 0.0778} & {\color[HTML]{1E1E1E} 0.47 ± 0.1453} & {\color[HTML]{1E1E1E} 0.75 ± 0.0474} & {\color[HTML]{1E1E1E} 0.58 ± 0.2581} & {\color[HTML]{1E1E1E} 0.71 ± 0.0586} & {\color[HTML]{1E1E1E} 0.76 ± 0.1219} \\ \hline
\end{tabular}
\end{table}
\end{landscape}

==> tables/comparision_f1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\centering
\caption{Comparison of  the F1 scores for the 3 approaches (Efficient-net b2)}
\label{tab:comparision_f1}
\begin{tabular}{ccccccc}
\hline
Approach                          & &   & \multirow{2}{*}{Train F1}& & & \multirow{2}{*}{Test F1} \\ \cline{1-1}
Pre-training method + train data   & &  &                         &  &  &                        \\ \hline
\hline
& & & \\
Supervised Imagenet + 80\%         & &  & 0.73 ± 0.007          &  &  & \textbf{0.72 ± 0.029}    \\ 
 & & & \\
Supervised Imagenet + 20\%        &  &  & 0.65 ±  0.061         &   &  & 0.54 ±  0.023            \\ 
& & & \\
Self-supervised Depth Contrast + 20\% & & & 0.71 ±  0.039        &   &  & \textbf{0.65 ±  0.026}   \\ 
\hline
\end{tabular}

\end{table}

==> tables/overall_F1_supervised.tex <==



\begin{table}[]
\centering
\caption{The F-1 score for supervised imagenet pre-trained and train on 80\% data (experiment 1a, 1b, and 1c)}
\label{tab:supervised_F1_overall}
\begin{tabular}{c c c  c c}
\hline
Network architecture & & Train F1     & & Test F1       \\ \hline
\hline
 & & & & \\
Efficient-net b2    & & 0.73 ± 0.0077 & & 0.72 ± 0.0294 \\
 & & & & \\
DenseNet 121      &  & 0.74 ± 0.0297 & & 0.72 ± 0.0411 \\
 & & & & \\
ResNeXt (31 x 4d)  &  & 0.75 ± 0.0321 & & 0.67 ± 0.0841 \\ \hline
\end{tabular}
\end{table}
